A Large-Scale Sensitivity Analysis on Latent Embeddings and Dimensionality Reductions for Text Spatializations

The semantic similarity between documents of a text corpus can be visualized using map-like metaphors based on two-dimensional scatterplot layouts. These layouts result from a dimensionality reduction on the document-term matrix or a representation within a latent embedding, including topic models. Thereby, the resulting layout depends on the input data and hyperparameters of the dimensionality reduction and is therefore affected by changes in them. Furthermore, the resulting layout is affected by changes in the input data and hyperparameters of the dimensionality reduction. However, such changes to the layout require additional cognitive efforts from the user. In this work, we present a sensitivity study that analyzes the stability of these layouts concerning (1) changes in the text corpora, (2) changes in the hyperparameter, and (3) randomness in the initialization. Our approach has two stages: data measurement and data analysis. First, we derived layouts for the combination of three text corpora and six text embeddings and a grid-search-inspired hyperparameter selection of the dimensionality reductions. Afterward, we quantified the similarity of the layouts through ten metrics, concerning local and global structures and class separation. Second, we analyzed the resulting 42817 tabular data points in a descriptive statistical analysis. From this, we derived guidelines for informed decisions on the layout algorithm and highlight specific hyperparameter settings. We provide our implementation as a Git repository at https://github.com/hpicgs/Topic-Models-and-Dimensionality-Reduction-Sensitivity-Study and results as Zenodo archive at https://doi.org/10.5281/zenodo.12772898.

==> tables-cached/correlation-matrix.tex <==
\begingroup \tiny %
\begin {tabular}{r>{\tiny }r>{\tiny }r>{\tiny }r>{\tiny }r>{\tiny }r>{\tiny }r@{\hspace {10pt}}>{\tiny }r>{\tiny }r>{\tiny }r@{\hspace {10pt}}>{\tiny }r>{\tiny }r@{\hspace {10pt}}>{\tiny }rc}%
\multicolumn {1}{c}{\strut }&\multicolumn {1}{c}{$\alpha _{T}$}&\multicolumn {1}{c}{$\alpha _{C}$}&\multicolumn {1}{c}{$\alpha _{MM}$}&\multicolumn {1}{c}{$\alpha _{MF}$}&\multicolumn {1}{c}{$\alpha _{LC}$}&\multicolumn {1}{c}{$\alpha _{LP}$}&\multicolumn {1}{c}{$\beta _{PC}$}&\multicolumn {1}{c}{$\beta _{SC}$}&\multicolumn {1}{c}{$\beta _{CO}$}&\multicolumn {1}{c}{$\gamma _{DC}$}&\multicolumn {1}{c}{$\gamma _{SC}$}&\multicolumn {1}{c}{$\theta _{PA}$}&\multicolumn {1}{c}{}\\%
\strut $\alpha _{T}$&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.06924,0.4727,0.70638}\definecolor {mapped color}{rgb}{0.06924,0.4727,0.70638}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.02219,0.44467,0.69102}\definecolor {mapped color}{rgb}{0.02219,0.44467,0.69102}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.07603,0.47675,0.7086}\definecolor {mapped color}{rgb}{0.07603,0.47675,0.7086}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.37914,0.65732,0.80748}\definecolor {mapped color}{rgb}{0.37914,0.65732,0.80748}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.46394,0.70784,0.83514}\definecolor {mapped color}{rgb}{0.46394,0.70784,0.83514}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.15918,0.52629,0.73573}\definecolor {mapped color}{rgb}{0.15918,0.52629,0.73573}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.14934,0.52042,0.73251}\definecolor {mapped color}{rgb}{0.14934,0.52042,0.73251}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.92229,0.94568,0.95715}\definecolor {mapped color}{rgb}{0.92229,0.94568,0.95715}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.96202,0.78859,0.71175}\definecolor {mapped color}{rgb}{0.96202,0.78859,0.71175}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96756,0.94,0.92778}\definecolor {mapped color}{rgb}{0.96756,0.94,0.92778}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96803,0.95247,0.94557}\definecolor {mapped color}{rgb}{0.96803,0.95247,0.94557}\pgfutilensuremath {0.0}&\multirow {\pgfplotstablerows }{*}{ \hspace *{-2.9cm} \begin {tikzpicture}[inner sep=0pt,outer sep=0pt] \begin {axis}[ hide axis, scale only axis, height=0cm, width=0cm, /pgfplots/colormap name=RdBu-5, colorbar horizontal, point meta min=-1, point meta max=1, colorbar style={ width=3.2cm, height=0.2cm, rotate=90, xtick style={draw=gray}, xtick={-1,-0.5,0,0.5,1}, xticklabels={$-1.0$,$-0.5$,\phantom {$-$}$0.0$,\phantom {$-$}$0.5$,\phantom {$-$}$1.0$}, xticklabel style={ font=\scriptsize , xshift=3pt, yshift=-0.2ex, anchor=west, }, typeset ticklabels with strut, at={(0.0,0.0)},anchor=south, }] \addplot [draw=none] coordinates {(0,0) (1,1)}; \end {axis} \end {tikzpicture} }\\%
\strut $\alpha _{C}$&\cellcolor [rgb]{0.06924,0.4727,0.70638}\definecolor {mapped color}{rgb}{0.06924,0.4727,0.70638}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.07649,0.47702,0.70874}\definecolor {mapped color}{rgb}{0.07649,0.47702,0.70874}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.02222,0.44469,0.69104}\definecolor {mapped color}{rgb}{0.02222,0.44469,0.69104}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.38025,0.65797,0.80785}\definecolor {mapped color}{rgb}{0.38025,0.65797,0.80785}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.4634,0.70753,0.83496}\definecolor {mapped color}{rgb}{0.4634,0.70753,0.83496}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.15732,0.52516,0.7351}\definecolor {mapped color}{rgb}{0.15732,0.52516,0.7351}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.14749,0.51932,0.7319}\definecolor {mapped color}{rgb}{0.14749,0.51932,0.7319}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.91852,0.94382,0.9562}\definecolor {mapped color}{rgb}{0.91852,0.94382,0.9562}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.96202,0.78825,0.71126}\definecolor {mapped color}{rgb}{0.96202,0.78825,0.71126}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96745,0.93687,0.92334}\definecolor {mapped color}{rgb}{0.96745,0.93687,0.92334}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96838,0.9622,0.95946}\definecolor {mapped color}{rgb}{0.96838,0.9622,0.95946}\pgfutilensuremath {0.0}&\\%
\strut $\alpha _{MM}$&\cellcolor [rgb]{0.02219,0.44467,0.69102}\definecolor {mapped color}{rgb}{0.02219,0.44467,0.69102}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.07649,0.47702,0.70874}\definecolor {mapped color}{rgb}{0.07649,0.47702,0.70874}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.08264,0.48068,0.71075}\definecolor {mapped color}{rgb}{0.08264,0.48068,0.71075}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.38454,0.66054,0.80923}\definecolor {mapped color}{rgb}{0.38454,0.66054,0.80923}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.47353,0.71355,0.83827}\definecolor {mapped color}{rgb}{0.47353,0.71355,0.83827}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.16762,0.5313,0.73846}\definecolor {mapped color}{rgb}{0.16762,0.5313,0.73846}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.15825,0.52573,0.73541}\definecolor {mapped color}{rgb}{0.15825,0.52573,0.73541}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.9219,0.9455,0.95705}\definecolor {mapped color}{rgb}{0.9219,0.9455,0.95705}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.96213,0.7912,0.71547}\definecolor {mapped color}{rgb}{0.96213,0.7912,0.71547}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.9677,0.94363,0.93297}\definecolor {mapped color}{rgb}{0.9677,0.94363,0.93297}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96799,0.95155,0.94426}\definecolor {mapped color}{rgb}{0.96799,0.95155,0.94426}\pgfutilensuremath {0.0}&\\%
\strut $\alpha _{MF}$&\cellcolor [rgb]{0.07603,0.47675,0.7086}\definecolor {mapped color}{rgb}{0.07603,0.47675,0.7086}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.02222,0.44469,0.69104}\definecolor {mapped color}{rgb}{0.02222,0.44469,0.69104}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.08264,0.48068,0.71075}\definecolor {mapped color}{rgb}{0.08264,0.48068,0.71075}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.3863,0.66159,0.80981}\definecolor {mapped color}{rgb}{0.3863,0.66159,0.80981}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.47266,0.71303,0.838}\definecolor {mapped color}{rgb}{0.47266,0.71303,0.838}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.16551,0.53006,0.73778}\definecolor {mapped color}{rgb}{0.16551,0.53006,0.73778}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.15613,0.52446,0.73473}\definecolor {mapped color}{rgb}{0.15613,0.52446,0.73473}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.91792,0.94353,0.95607}\definecolor {mapped color}{rgb}{0.91792,0.94353,0.95607}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.96213,0.79138,0.71573}\definecolor {mapped color}{rgb}{0.96213,0.79138,0.71573}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96759,0.94063,0.92868}\definecolor {mapped color}{rgb}{0.96759,0.94063,0.92868}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96844,0.96388,0.96187}\definecolor {mapped color}{rgb}{0.96844,0.96388,0.96187}\pgfutilensuremath {0.0}&\\%
\strut $\alpha _{LC}$&\cellcolor [rgb]{0.37914,0.65732,0.80748}\definecolor {mapped color}{rgb}{0.37914,0.65732,0.80748}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.38025,0.65797,0.80785}\definecolor {mapped color}{rgb}{0.38025,0.65797,0.80785}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.38454,0.66054,0.80923}\definecolor {mapped color}{rgb}{0.38454,0.66054,0.80923}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.3863,0.66159,0.80981}\definecolor {mapped color}{rgb}{0.3863,0.66159,0.80981}\pgfutilensuremath {0.7}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.53613,0.75085,0.8587}\definecolor {mapped color}{rgb}{0.53613,0.75085,0.8587}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.41844,0.68074,0.8203}\definecolor {mapped color}{rgb}{0.41844,0.68074,0.8203}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.40973,0.67554,0.81747}\definecolor {mapped color}{rgb}{0.40973,0.67554,0.81747}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.92438,0.94672,0.95766}\definecolor {mapped color}{rgb}{0.92438,0.94672,0.95766}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.96402,0.84314,0.78957}\definecolor {mapped color}{rgb}{0.96402,0.84314,0.78957}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.9652,0.8753,0.83546}\definecolor {mapped color}{rgb}{0.9652,0.8753,0.83546}\pgfutilensuremath {-0.1}&\cellcolor [rgb]{0.96848,0.96481,0.9632}\definecolor {mapped color}{rgb}{0.96848,0.96481,0.9632}\pgfutilensuremath {0.0}&\\%
\vspace {5pt}\strut $\alpha _{LP}$&\cellcolor [rgb]{0.46394,0.70784,0.83514}\definecolor {mapped color}{rgb}{0.46394,0.70784,0.83514}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.4634,0.70753,0.83496}\definecolor {mapped color}{rgb}{0.4634,0.70753,0.83496}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.47353,0.71355,0.83827}\definecolor {mapped color}{rgb}{0.47353,0.71355,0.83827}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.47266,0.71303,0.838}\definecolor {mapped color}{rgb}{0.47266,0.71303,0.838}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.53613,0.75085,0.8587}\definecolor {mapped color}{rgb}{0.53613,0.75085,0.8587}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.56638,0.76886,0.86856}\definecolor {mapped color}{rgb}{0.56638,0.76886,0.86856}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.55295,0.76086,0.86418}\definecolor {mapped color}{rgb}{0.55295,0.76086,0.86418}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.8676,0.91861,0.94362}\definecolor {mapped color}{rgb}{0.8676,0.91861,0.94362}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.95706,0.65274,0.5179}\definecolor {mapped color}{rgb}{0.95706,0.65274,0.5179}\pgfutilensuremath {-0.5}&\cellcolor [rgb]{0.9645,0.85602,0.80795}\definecolor {mapped color}{rgb}{0.9645,0.85602,0.80795}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.96805,0.95306,0.94643}\definecolor {mapped color}{rgb}{0.96805,0.95306,0.94643}\pgfutilensuremath {0.0}&\\%
\strut $\beta _{PC}$&\cellcolor [rgb]{0.15918,0.52629,0.73573}\definecolor {mapped color}{rgb}{0.15918,0.52629,0.73573}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.15732,0.52516,0.7351}\definecolor {mapped color}{rgb}{0.15732,0.52516,0.7351}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.16762,0.5313,0.73846}\definecolor {mapped color}{rgb}{0.16762,0.5313,0.73846}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.16551,0.53006,0.73778}\definecolor {mapped color}{rgb}{0.16551,0.53006,0.73778}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.41844,0.68074,0.8203}\definecolor {mapped color}{rgb}{0.41844,0.68074,0.8203}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.56638,0.76886,0.86856}\definecolor {mapped color}{rgb}{0.56638,0.76886,0.86856}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.0234,0.44539,0.69142}\definecolor {mapped color}{rgb}{0.0234,0.44539,0.69142}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.70305,0.83714,0.90288}\definecolor {mapped color}{rgb}{0.70305,0.83714,0.90288}\pgfutilensuremath {0.3}&\cellcolor [rgb]{0.95998,0.73251,0.63171}\definecolor {mapped color}{rgb}{0.95998,0.73251,0.63171}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.96454,0.85704,0.8094}\definecolor {mapped color}{rgb}{0.96454,0.85704,0.8094}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.96806,0.95341,0.94693}\definecolor {mapped color}{rgb}{0.96806,0.95341,0.94693}\pgfutilensuremath {0.0}&\\%
\strut $\beta _{SC}$&\cellcolor [rgb]{0.14934,0.52042,0.73251}\definecolor {mapped color}{rgb}{0.14934,0.52042,0.73251}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.14749,0.51932,0.7319}\definecolor {mapped color}{rgb}{0.14749,0.51932,0.7319}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.15825,0.52573,0.73541}\definecolor {mapped color}{rgb}{0.15825,0.52573,0.73541}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.15613,0.52446,0.73473}\definecolor {mapped color}{rgb}{0.15613,0.52446,0.73473}\pgfutilensuremath {0.9}&\cellcolor [rgb]{0.40973,0.67554,0.81747}\definecolor {mapped color}{rgb}{0.40973,0.67554,0.81747}\pgfutilensuremath {0.6}&\cellcolor [rgb]{0.55295,0.76086,0.86418}\definecolor {mapped color}{rgb}{0.55295,0.76086,0.86418}\pgfutilensuremath {0.5}&\cellcolor [rgb]{0.0234,0.44539,0.69142}\definecolor {mapped color}{rgb}{0.0234,0.44539,0.69142}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.71999,0.84554,0.90707}\definecolor {mapped color}{rgb}{0.71999,0.84554,0.90707}\pgfutilensuremath {0.3}&\cellcolor [rgb]{0.95996,0.73236,0.6315}\definecolor {mapped color}{rgb}{0.95996,0.73236,0.6315}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.96463,0.85959,0.81305}\definecolor {mapped color}{rgb}{0.96463,0.85959,0.81305}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.96808,0.9539,0.94763}\definecolor {mapped color}{rgb}{0.96808,0.9539,0.94763}\pgfutilensuremath {0.0}&\\%
\vspace {5pt}\strut $\beta _{CO}$&\cellcolor [rgb]{0.92229,0.94568,0.95715}\definecolor {mapped color}{rgb}{0.92229,0.94568,0.95715}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.91852,0.94382,0.9562}\definecolor {mapped color}{rgb}{0.91852,0.94382,0.9562}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.9219,0.9455,0.95705}\definecolor {mapped color}{rgb}{0.9219,0.9455,0.95705}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.91792,0.94353,0.95607}\definecolor {mapped color}{rgb}{0.91792,0.94353,0.95607}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.92438,0.94672,0.95766}\definecolor {mapped color}{rgb}{0.92438,0.94672,0.95766}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.8676,0.91861,0.94362}\definecolor {mapped color}{rgb}{0.8676,0.91861,0.94362}\pgfutilensuremath {0.1}&\cellcolor [rgb]{0.70305,0.83714,0.90288}\definecolor {mapped color}{rgb}{0.70305,0.83714,0.90288}\pgfutilensuremath {0.3}&\cellcolor [rgb]{0.71999,0.84554,0.90707}\definecolor {mapped color}{rgb}{0.71999,0.84554,0.90707}\pgfutilensuremath {0.3}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.95738,0.66193,0.531}\definecolor {mapped color}{rgb}{0.95738,0.66193,0.531}\pgfutilensuremath {-0.5}&\cellcolor [rgb]{0.9597,0.72488,0.62083}\definecolor {mapped color}{rgb}{0.9597,0.72488,0.62083}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.96767,0.94296,0.932}\definecolor {mapped color}{rgb}{0.96767,0.94296,0.932}\pgfutilensuremath {0.0}&\\%
\strut $\gamma _{DC}$&\cellcolor [rgb]{0.96202,0.78859,0.71175}\definecolor {mapped color}{rgb}{0.96202,0.78859,0.71175}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96202,0.78825,0.71126}\definecolor {mapped color}{rgb}{0.96202,0.78825,0.71126}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96213,0.7912,0.71547}\definecolor {mapped color}{rgb}{0.96213,0.7912,0.71547}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96213,0.79138,0.71573}\definecolor {mapped color}{rgb}{0.96213,0.79138,0.71573}\pgfutilensuremath {-0.3}&\cellcolor [rgb]{0.96402,0.84314,0.78957}\definecolor {mapped color}{rgb}{0.96402,0.84314,0.78957}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.95706,0.65274,0.5179}\definecolor {mapped color}{rgb}{0.95706,0.65274,0.5179}\pgfutilensuremath {-0.5}&\cellcolor [rgb]{0.95998,0.73251,0.63171}\definecolor {mapped color}{rgb}{0.95998,0.73251,0.63171}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.95996,0.73236,0.6315}\definecolor {mapped color}{rgb}{0.95996,0.73236,0.6315}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.95738,0.66193,0.531}\definecolor {mapped color}{rgb}{0.95738,0.66193,0.531}\pgfutilensuremath {-0.5}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.2568,0.58443,0.76756}\definecolor {mapped color}{rgb}{0.2568,0.58443,0.76756}\pgfutilensuremath {0.8}&\cellcolor [rgb]{0.94963,0.95921,0.96391}\definecolor {mapped color}{rgb}{0.94963,0.95921,0.96391}\pgfutilensuremath {0.0}&\\%
\vspace {5pt}\strut $\gamma _{SC}$&\cellcolor [rgb]{0.96756,0.94,0.92778}\definecolor {mapped color}{rgb}{0.96756,0.94,0.92778}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96745,0.93687,0.92334}\definecolor {mapped color}{rgb}{0.96745,0.93687,0.92334}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.9677,0.94363,0.93297}\definecolor {mapped color}{rgb}{0.9677,0.94363,0.93297}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96759,0.94063,0.92868}\definecolor {mapped color}{rgb}{0.96759,0.94063,0.92868}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.9652,0.8753,0.83546}\definecolor {mapped color}{rgb}{0.9652,0.8753,0.83546}\pgfutilensuremath {-0.1}&\cellcolor [rgb]{0.9645,0.85602,0.80795}\definecolor {mapped color}{rgb}{0.9645,0.85602,0.80795}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.96454,0.85704,0.8094}\definecolor {mapped color}{rgb}{0.96454,0.85704,0.8094}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.96463,0.85959,0.81305}\definecolor {mapped color}{rgb}{0.96463,0.85959,0.81305}\pgfutilensuremath {-0.2}&\cellcolor [rgb]{0.9597,0.72488,0.62083}\definecolor {mapped color}{rgb}{0.9597,0.72488,0.62083}\pgfutilensuremath {-0.4}&\cellcolor [rgb]{0.2568,0.58443,0.76756}\definecolor {mapped color}{rgb}{0.2568,0.58443,0.76756}\pgfutilensuremath {0.8}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\cellcolor [rgb]{0.96223,0.96545,0.96704}\definecolor {mapped color}{rgb}{0.96223,0.96545,0.96704}\pgfutilensuremath {0.0}&\\%
\strut $\theta _{PA}$&\cellcolor [rgb]{0.96803,0.95247,0.94557}\definecolor {mapped color}{rgb}{0.96803,0.95247,0.94557}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96838,0.9622,0.95946}\definecolor {mapped color}{rgb}{0.96838,0.9622,0.95946}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96799,0.95155,0.94426}\definecolor {mapped color}{rgb}{0.96799,0.95155,0.94426}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96844,0.96388,0.96187}\definecolor {mapped color}{rgb}{0.96844,0.96388,0.96187}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96848,0.96481,0.9632}\definecolor {mapped color}{rgb}{0.96848,0.96481,0.9632}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96805,0.95306,0.94643}\definecolor {mapped color}{rgb}{0.96805,0.95306,0.94643}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96806,0.95341,0.94693}\definecolor {mapped color}{rgb}{0.96806,0.95341,0.94693}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96808,0.9539,0.94763}\definecolor {mapped color}{rgb}{0.96808,0.9539,0.94763}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96767,0.94296,0.932}\definecolor {mapped color}{rgb}{0.96767,0.94296,0.932}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.94963,0.95921,0.96391}\definecolor {mapped color}{rgb}{0.94963,0.95921,0.96391}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.96223,0.96545,0.96704}\definecolor {mapped color}{rgb}{0.96223,0.96545,0.96704}\pgfutilensuremath {0.0}&\cellcolor [rgb]{0.02083,0.44386,0.69058}\definecolor {mapped color}{rgb}{0.02083,0.44386,0.69058}\pgfutilensuremath {1.0}&\\%
\end {tabular}%
\endgroup %

